Efficient Auxiliary-Field Quantum Monte Carlo using Isometric Tensor Hypercontraction

Auxiliary Field Quantum Monte Carlo (AFQMC) has emerged as a powerful framework for treating strongly correlated electronic systems, offering a favorable balance between computational cost and accuracy. In this paper, we present a novel AFQMC method that uses the isometric tensor hypercontraction (ITHC) technique to diagonalize the two-body Coulomb interaction of molecular electronic Hamiltonians by introducing additional fictitious fermionic modes. Our method shows reduced theoretical complexity and better practical performance for both propagation and local energy evaluation compared to the standard AFQMC method. We demonstrate the efficacy of this approach by computing the ground-state energies of a linear $\ce{H10}$-chain and the benzene molecule. Our results show that the extended-basis AFQMC recovers many-body correlations with a precision comparable to that of high-level wavefunction methods such as Coupled Clusters (CC) or Density Matrix Renormalization Group (DMRG), while offering significantly improved scaling.

==> implementation_bkp.tex <==
\section{IMPLEMENTATIONAL DETAILS}
\label{sec:implementation}

In this section, we describe the implementation details of our extended basis AFQMC method. To implement our extended basis AFQMC propagator, we utilised the Python package ipie by Joonho Lee et al. \cite{Malone.2023} as a basis and added an additional propagator and other functionalities.


\subsection{Enlarged Basis Propagator}
We implement the propagator given in Eq.(\ref{Extended propagator}) in the extended basis set. Since we are using single Slater-determinant states, the application of the imaginary-time propagator in Eq.(\ref{Extended propagator}) can be performed as a simple matrix-matrix multiplication. After applying the one-body propagator in the original basis with dimension $N$, the trial and walker determinant matrices $A$ and $B$ with dimension $(N,N_e)$, are half rotated as
\begin{align}
\label{half-rotation}
       \tilde{A}_{\alpha k}= \sum_{i=1}^{N} u_{i \alpha} A_{ik}\\
       \tilde{B}_{\alpha k}= \sum_{i=1}^{N} u_{i\alpha} B_{ik}.
\end{align}
\noindent Here $u_{i \alpha}$ is an isometry. The half-rotation of the Slater determinant, as stated in Eq. (\ref{half-rotation}), can be done at a cost of $\mathcal{O}(N_{walkers}MNN_e)$. This allows us to apply the two-body propagator in the extended basis as
\begin{align}
     e^{x \sqrt{- \Delta \tau} \hat{v}} \ket{\phi}= \sum_{\alpha} (e^{x \sqrt{- \Delta \tau}\hat{v}})_{\alpha} \tilde{B}_{\alpha k},
\end{align}
\noindent for each auxiliary field configuration $x$. Since the two-body interaction term is diagonal in the extended space, this can be done at a cost of $\mathcal{O}(N_{walkers}MN_e)$.
\begin{algorithm}
\caption{Two-body propagation}
\begin{algorithmic}
\State $\mathbf{Input:}$ Initial batch of walkers $\{ \ket{\phi_{w}} \}$ as Slater-determinants

\State $\mathbf{Output:}$ Propagated walkers $\mathbf{P} e^{-\Delta \tau \hat{W}}\mathbf{P} \ket{\phi_{w}}$
\For{each walker $w = 1, \dots, N_{walkers}$}
\State Half-rotation of walkers: $\ket{\tilde{\phi}_w}=U \ket{\phi_w}$
\State Set up two-body propagator
\For{$\alpha = 1, \dots, M$}
\State Sample a random auxiliary field $x_{\alpha}$ from $p(x)$
\EndFor
\State Apply two-body propagator $e^{T(x)}$
\State $\ket{\tilde{\phi}_w^{'}}=e^{T(x)} \ket{\tilde{\phi}_w}$
\State Rotate back to original space: $\ket{\phi_w^{'}}=U^{-1} \ket{\tilde{\phi}_w^{'}}$
\EndFor
\end{algorithmic}
\end{algorithm}
\noindent Before and after the application of the two-body propagator, the walkers are propagated via the one-body term in the original basis set. 

\subsection{One-body Green's function and force bias}
To calculate expectation values of observables and the dynamical force bias, the one-body Green's function is calculated in the enlarged basis
\begin{align}
   \expval{n_{\alpha}} = \sum_{ij} \frac{\mel{\Psi_{trial}}{u_{\alpha i} \hat{a}_i^{\dagger} \hat{a}_j u_{j \alpha}}{\Psi}}{\braket{\Psi_{trial}}{\Psi}}= \sum_{ij} u_{\alpha i} u_{j \alpha} G_{ij} .
\end{align}
\noindent For single Slater determinant trial states and walkers, the one-body Green's function in the original basis $G_{ij}$ can be written as $A^*(B^TA)^{-1}B^T=A^* G^{half}$, where $A$ and $B$ are Slater determinant matrices of trial state and walker state, respectively. A more efficient computation of the transformed one-body Green's function can be achieved by first performing a half-rotation of the trial state and walkers, like in Eq.(\ref{half-rotation}). This enables the calculation of the Green's function with a theoretical complexity of $\mathcal{O}(N_{walkers}MN_e^2)$. 
\begin{algorithm}
\caption{Construction of half-rotated Green's function}
\begin{algorithmic}
\State $\mathbf{Input:}$ Trial $\ket{\Psi_T}$ and walker batch $\{\ket{\phi_w} \}$ as Slater-determinant matrices A and B

\State $\mathbf{Output:}$ Green's function in extended basis $\expval{n_{\alpha}}$
\For{each walker $w = 1, \dots, N_{walkers}$} 
\State Inverse Overlap= $(B^T_w A)^{-1}$ 
\State $G_{Half,w}$= Inverse Overlap $\cdot B^T_w$
\State $\expval{n_{\alpha ,w}}$=  $A^* \cdot G_{Half,w}$
\EndFor
\end{algorithmic}

\end{algorithm}
\noindent The dynamic force bias can then be calculated via a dot product at a cost of $\mathcal{O}(N_{walkers}M)$.

%\begin{align}
%    \Bar{v}= \sum_i \expval{n_{i}} \hat{v}_i
%\end{align}

\subsection{Energy estimator}
The local energy is determined via the mixed estimator
\begin{align}
    E_w= \frac{\mel{\Psi_{trial}}{\hat{H}}{\phi_w}}{\braket{\Psi_{trial}}{\phi_w}}
\end{align}
\noindent For Slater-determinant states, this can be done via the one-particle Green's function. While the one-body energy is evaluated in the original space, we evaluate the two-body interaction energy in the extended space 
\begin{align}
    \expval{V}= \sum_{ij} W_{ij} (\tilde{G}_{ii} \tilde{G}_{jj}- \tilde{G}_{ij} \tilde{G}_{ji}),
\end{align}
where $\tilde{G}_{ij}$ is the Green's function in the extended basis and $W_{ij}$ is the transformed ERI in the extended space representation.
\begin{algorithm}
\caption{Extended space energy estimator}
\begin{algorithmic}
\State $\mathbf{Input:}$ Trial $\ket{\Psi_T}$ and walker batch $\{\ket{\phi_w} \}$ as Slater-determinant matrices A and B

\State $\mathbf{Output:}$ Total energy $\expval{E_{total}}$
\For{each walker $w = 1, \dots, N_{walkers}$}
\EndFor
\end{algorithmic}

\end{algorithm}


\subsection{Mean-Field Shift}
A mean-field shift was calculated according to Eq. (\ref{mean field shift}). Due to the Hubbard-like nature of the interaction term, the mean-field can be evaluated as a simple dot product using the single-particle Green's function in the extended space. For every walker the mean-field shift is calculated as
\begin{align}
    \bar{v}= \sum_{\alpha} v_{\alpha} \expval{n_{ \alpha}}.
\end{align}
